Multimodal vs. Unimodal Physiological Control in Videogames for Enhanced Realism and Depth

(arXiv abridged abstract) In the last two decades, videogames have evolved in a nearly explosive way from the pixelated graphics to today's near-realistic 3D environments. The interaction devices traditionally used in videogames have not evolved with the same intensity, but recent HCI studies have explored biofeedback interaction - the explicit manipulation of a person's physiological data as input to a system - as an alternative to them. Traditional biofeedback prototypes apply 1 sensor to each game mechanic (unimodality). In this dissertation, we introduce the combination of 2 physiological sensors simultaneously per game mechanic (multimodality) and present a First-Person Shooter game comprised of 8 game mechanics with three interaction flavours (no biofeedback/vanilla, unimodal and multimodal). An empirical study with 32 regular players was employed to explore and study differences between the three interaction types and where they can be best employed. Players compared the three games in terms of Fun, Ease of Use, Originality, Playability and Favourite Condition. For the sake of completeness, other evaluation methods were used as well: IMI Questionnaire, keywords association and open-ended commentaries. The vanilla version was considered easier to use, but both biofeedback versions were considered the most fun. Both versions were praised differently: the unimodal version for its simplicity of use, and the multimodal for its realism, activation safety of game mechanics and depth added to the game. Our conclusion is that multimodal biofeedback can have a relevant impact in terms of added depth, depending on the way it is used inside the game. On a boundary case, it can be used to increase the feeling of empowerment on the player when using certain abilities, or to intentionally make in-game actions more difficult by demanding more physical effort from the player.

==> Makefile <==
#
# Makefile for feupteses/feupthesis
#
# Version:   Sat May 17 22:36:50 2008
# Written by JCL
#

## programs
LATEX=latex
PDFLATEX=pdflatex
BIBTEX=bibtex
DVIDVI=dvidvi -m '2:0(3mm,-14mm),1(193mm,-14mm)'
DVIPS=dvips -Ppdf
DVI2PS=dvips -t landscape -x 707
PS2PDF=ps2pdf -dEmbedAllFonts#true
MKIDX=makeindex

## Basename for result in PT
TARGET=mieic
## Basename for result in EN
#TARGET=mieic-en

## Basename for PDIS
#TARGET=pdis
#TARGET=pdis-en

## .tex files
TEXFILES=$(wildcard *.tex **/*.tex)

## BibTeX files
BIB=$(wildcard *.bib)

## paper
PAPERSIZE=a4

#we prefer pdflatex for bibtex
LATEXBIB=$(PDFLATEX)

main:	$(TARGET).pdf

index:
	$(MKIDX) $(TARGET)

biblio:
	$(BIBTEX) $(TARGET)

.tex.pdf:
	rm -f $(TARGET).pdf
	$(PDFLATEX) $< $@ || { rm -f $*.aux $*.idx && false ; }
	if grep 'There were undefined references' $*.log ; then \
	  $(BIBTEX) $(TARGET); $(PDFLATEX) $< $@; fi
	while grep 'Rerun to get cross-references right.' $*.log ; do \
	  $(PDFLATEX) $< $@ || { rm -f $*.aux $*.idx && false ; } ; done

.tex.dvi:
	rm -f $*.ps $*.pdf
	$(LATEX) $< || { rm -f $*.dvi $*.aux $*.idx && false ; }
	if grep 'There were undefined references' $*.log ; then \
	  $(BIBTEX) $(TARGET); $(LATEX) $< $@; fi
	while grep 'Rerun to get cross-references right.' $*.log ; do \
	  $(LATEX) $< || { rm -f $*.dvi $*.aux $*.idx && false ; } ; done

.dvi.ps:
	$(DVIPS) -t $(PAPERSIZE) $< -o $@

.dvi.dvi2:
	$(DVIDVI) $< $@

.dvi2.ps2:
	$(DVI2PS) $< -o $@

.ps.pdf:
	$(PS2PDF) $< $@

.bib.bbl:
# in case we don't already have a .aux file listing citations
	$(LATEXBIB) $(TARGET).tex
# get the citations out of the bibliography
	$(BIBTEX) $(TARGET)
# do it again in case there are out-of-order cross-references
	$(LATEXBIB) $(TARGET).tex
	$(BIBTEX) $(TARGET)

$(TARGET).pdf:	  $(TEXFILES)
$(TARGET).dvi:	  $(TEXFILES)
$(TARGET).ps:	  $(TARGET).dvi
$(TARGET).ps2:	  $(TARGET).dvi2
$(TARGET).dvi2:	  $(TARGET).dvi

## Extensions
EXTS=aux toc idx ind ilg log out lof lot lol bbl blg

##clean
clean:
	for EXT in ${EXTS}; do \
	  find `pwd` -name \*\.$${EXT} -exec rm -v \{\} \; ; done

##show PDF
display: $(TARGET).pdf
	acroread $(TARGET).pdf &

### misc
.SUFFIXES: .tex .aux .toc .lof .lot .log .dvi .dvi2 .ps .ps2 .pdf .bib .bbl


==> acknows.tex <==
\chapter*{Agradecimentos}
%\addcontentsline{toc}{chapter}{Agradecimentos}

Aliquam id dui. Nulla facilisi. Nullam ligula nunc, viverra a, iaculis
at, faucibus quis, sapien. Cum sociis natoque penatibus et magnis dis
parturient montes, nascetur ridiculus mus. Curabitur magna ligula,
ornare luctus, aliquam non, aliquet at, tortor. Donec iaculis nulla
sed eros. Sed felis. Nam lobortis libero. Pellentesque
odio. Suspendisse potenti. Morbi imperdiet rhoncus magna. Morbi
vestibulum interdum turpis. Pellentesque varius. Morbi nulla urna,
euismod in, molestie ac, placerat in, orci. 

Ut convallis. Suspendisse luctus pharetra sem. Sed sit amet mi in diam
luctus suscipit. Nulla facilisi. Integer commodo, turpis et semper
auctor, nisl ligula vestibulum erat, sed tempor lacus nibh at
turpis. Quisque vestibulum pulvinar justo. Class aptent taciti
sociosqu ad litora torquent per conubia nostra, per inceptos
himenaeos. Nam sed tellus vel tortor hendrerit pulvinar. Phasellus
eleifend, augue at mattis tincidunt, lorem lorem sodales arcu, id
volutpat risus est id neque. Phasellus egestas ante. Nam porttitor
justo sit amet urna. Suspendisse ligula nunc, mollis ac, elementum
non, venenatis ut, mauris. Mauris augue risus, tempus scelerisque,
rutrum quis, hendrerit at, nunc. Nulla posuere porta orci. Nulla dui. 

Fusce gravida placerat sem. Aenean ipsum diam, pharetra vitae, ornare
et, semper sit amet, nibh. Nam id tellus. Etiam ultrices. Praesent
gravida. Aliquam nec sapien. Morbi sagittis vulputate dolor. Donec
sapien lorem, laoreet egestas, pellentesque euismod, porta at,
sapien. Integer vitae lacus id dui convallis blandit. Mauris non
sem. Integer in velit eget lorem scelerisque vehicula. Etiam tincidunt
turpis ac nunc. Pellentesque a justo. Mauris faucibus quam id
eros. Cras pharetra. Fusce rutrum vulputate lorem. Cras pretium magna
in nisl. Integer ornare dui non pede. 

\vspace{10mm}
\flushleft{O Nome do Autor}

